Structure Exploiting Interior Point Methods

Interior point methods are among the most popular techniques for large scale nonlinear optimization, owing to their intrinsic ability of scaling to arbitrary large problem sizes. Their efficiency has attracted in recent years a lot of attention due to increasing demand for large scale optimization in industry and engineering. A parallel interior point method is discussed that exploits the intrinsic structure of large-scale nonlinear optimization problems so that the solution process can employ massively parallel high-performance computing infastructures. Since the overall performance of interior point methods relies heavily on scalable sparse linear algebra solvers, particular emphasis is given to the underlying algorithms for the distributed solution of the associated sparse linear systems obtained at each iteration from the linearization of the optimality conditions. The interior point algorithm is implemented in a object-oriented parallel IPM solver and applied for the solution of large scale optimal control problems solved in a daily basis for the secure transmission and distribution of electricity in modern power grids.

==> CasesBenchmark.tex <==
% \newcommand\offone{-8.0ex}
% \newcommand\offtwo{-10.5ex}
% \newcommand\offthree{-4.5ex}

\begin{tikzpicture}[scale=1.0]

\begin{axis}
[
    separate axis lines,
    ymajorgrids,
    yminorgrids,
    minor tick num=0,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    ybar=2pt,
    bar width=4pt,
    width=\columnwidth,
    %xmin=1,
    ymin=1,
    %axis on top,
    ymax=1e6,
    xtick=data,
    ymode=log,   
    yminorticks=true,
    enlarge x limits=0.1,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={IEEE30I,IEEE30II,PEGASE1354I,PEGASE1354II,PEGASE13659I,PEGASE13659II},
    %symbolic x coords={IEEE30,PEGASE1354,PEGASE13659},
    %symbolic x coords={240,480,720,960,1200,1440,1680,1920,2160,2400,2640,2880},
    restrict y to domain*=1:1e7, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    %nodes near coords={ \pgfmathprintnumber{\rawy} },
    axis lines*=left,
    clip=false,
    %xticklabel style={font=\scriptsize},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xticklabel style={rotate=15,anchor=mid east, font=\scriptsize},
    axis background/.style={fill=none},
    legend style={at={(0.3,1)},legend cell align=left,align=left,draw=none,fill=none, font=\scriptsize},
    ylabel={Time (s)}
]
\addplot[fill=mycolor1]                                        table [x=Case, y=AveragePerIter]{data/runcases-HYPEROPT.dat};     \addlegendentry{MPFOPT}
\addplot[fill=mycolor2,postaction={pattern=horizontal lines}]  table [x=Case, y=AveragePerIter]{data/runcases-HYPEROPTmem.dat};  \addlegendentry{MPFOPTmem}
\addplot[fill=mycolor3,postaction={pattern=crosshatch}]        table [x=Case, y=AveragePerIter]{data/runcases-IPOPT.dat};        \addlegendentry{IPOPT}
\addplot[fill=mycolor4,postaction={pattern=north east lines}]  table [x=Case, y=Factorization]{data/runcasesMIPS-MIPS.dat};      \addlegendentry{MIPS}
\addplot[fill=mycolor5,postaction={pattern=north west lines}]  table [x=Case, y=AveragePerIter]{data/runcasesKNITRO-KNITRO.dat}; \addlegendentry{KNITRO}
\end{axis}
\end{tikzpicture}



==> figures/tab_slackElimination.tex <==
%tweak the space between columns, default is 6pt
\setlength{\tabcolsep}{10pt}

%set a fontsize (\small, \tiny, etc.) before the \begin{tabular}, then all cells will have this fontsize
\small

%G is a custom column with gray background, defined in preamble
\begin{tabular}{l r r G r r G}
& \multicolumn{3}{c}{\textbf{Peak Memory [GB]} }  & \multicolumn{3}{c}{\textbf{Solution Time [$s$]} }\\ 
\cmidrule(l{2pt}r{4pt}){2-4} \cmidrule(l{4pt}r{2pt}){5-7}
\multicolumn{1}{c}{\textbf{Benchmark}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}} \\ \midrule
%
\multicolumn{1}{l}{\footnotesize{PEGASE1354}} & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
\multicolumn{1}{l}{\footnotesize{PEGASE2869}} & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
\multicolumn{1}{l}{\footnotesize{PEGASE9241}} & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
\multicolumn{1}{l}{\footnotesize{ACTIVSg10k}} & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
\multicolumn{1}{l}{\footnotesize{PEGASE13659}} & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\
\end{tabular}

%return to normal fontsize
\normalsize


%%%% table with Nrows, Memory and Time statistic
% %G is a custom column with gray background, defined in preamble
% \begin{tabular}{l r r G r r G r r G}
% \toprule
% & \multicolumn{3}{c}{\textbf{Nrows $A_i$}}  & \multicolumn{3}{c}{\textbf{Peak Memory [GB]} }  & \multicolumn{3}{c}{\textbf{Solution Time [$s$]} }\\ 
% \cmidrule(l{2pt}r{4pt}){2-4} \cmidrule(l{4pt}r{2pt}){5-7} \cmidrule(l{4pt}r{2pt}){8-10}
% \multicolumn{1}{c}{\textbf{Benchmark}}           & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
% & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
% & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}} \\ \midrule
% %
% \multicolumn{1}{l}{\scriptsize{PEGASE1354}} & 13,899 & 9,971 & 28.65 & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
% \multicolumn{1}{l}{\scriptsize{PEGASE2869}} & 30,823 & 21,659 & 29.73 & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE9241}} & 104,049 & 71,951 & 30.85 & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k}} & 94,697 & 69,285 & 26.84 & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659}} & 144,687 & 103,753 & 28.29 & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\
% \bottomrule
% \end{tabular}

%%%%Full set of results. Above we show only the better of the MDO/Metis variants and do not further discuss this in the text.
% \multicolumn{1}{l}{\scriptsize{PEGASE1354}} & 13,899 & 9,971 & 28.65 & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
% \multicolumn{1}{l}{\scriptsize{PEGASE2869}} & 30,823 & 21,659 & 29.73 & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE9241}} & 104,049 & 71,951 & 30.85 & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k-Metis4}} & 94,697 & 69,285 & 26.84 & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k-MDO}} & 94,697 & 69,285 & 26.84 & 0.109 & 0.101 & 7.29 & 0.899 & 0.848 & 5.73 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659-Metis4}} & 144,687 & 103,753 & 28.29 & 0.326 & 0.316 & 3.07 & 2.029 & 2.256 & -11.22 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659-MDO}} & 144,687 & 103,753 & 28.29 & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\
